Approximate Max-Flow Min-Multicut Theorem for Graphs of Bounded Treewidth

We prove an approximate max-multiflow min-multicut theorem for bounded treewidth graphs. In particular, we show the following: Given a treewidth-$r$ graph, there exists a (fractional) multicommodity flow of value $f$, and a multicut of capacity $c$ such that $ f \leq c \leq \mathcal{O}(\ln (r+1)) \cdot f$. It is well known that the multiflow-multicut gap on an $r$-vertex (constant degree) expander graph can be $\Omega(\ln r)$, and hence our result is tight up to constant factors. Our proof is constructive, and we also obtain a polynomial time $\mathcal{O}(\ln (r+1))$-approximation algorithm for the minimum multicut problem on treewidth-$r$ graphs. Our algorithm proceeds by rounding the optimal fractional solution to the natural linear programming relaxation of the multicut problem. We introduce novel modifications to the well-known region growing algorithm to facilitate the rounding while guaranteeing at most a logarithmic factor loss in the treewidth.

==> extra_stuff.tex <==
\section{$(\alpha,\beta)$-Cover of Graphs}
Let $G=(V,E)$ be a graph with edge length $l:E \rightarrow \mathbb{R}_{\geq 0}$ and  $\alpha,\beta \in \mathbb{R}_{\geq 0}$. Given a set $S \subseteq V$, let $\textsc{dia}(S)=\max_{u,v \in S} d_{G}(u,v)$. Given two sets $S,T \subseteq V$, let $d(S,T)=\min_{u \in S, v \in T}d_G(u,v)$. Let $\mathcal{S}=\{S_1,S_2,\ldots,S_m\}$ be a collection disjoint subsets of $V$. $\mathcal{S}$ is called $(\alpha,\beta)$-good if $\textsc{dia}(S_i) \leq \alpha$ and $d(S_i,S_j) \geq \beta$ for each $1 \leq i \neq j \leq m$. Let $\textsc{cov}(\mathcal{S})=\cup_{i=1}^{m} S_i$. A collection $\mathcal{S}_1,\mathcal{S}_2,\ldots,\mathcal{S}_k$ of $(\alpha,\beta)$-good sets is called a $(\alpha,\beta)$-Cover of $G$ if $\cup _{i=1}^{k} \textsc{cov}({S}_i)=V$. We say that $G$ has $(\alpha,\beta)$-Cover of size $k$. We will prove the following theorems, which together show that graph of width $r$ have a small-diameter decomposition of low cost.

\begin{theorem}
Let $G=(V,E)$ be a graph with edge capacities $c:E \rightarrow \mathbb{R}_{\geq 0}$ and edge lengths $l: E \rightarrow \mathbb{R}_{\geq 0}$. If there exists a $(1/2,1/4)$-cover of $G$ of size $k$, then there exists a small diameter decomposition of $G$ with cost at most $8 \cdot \log (k+1) \cdot F$, where $F=\sum_{e \in E}c(e) \cdot l(e)$.
\end{theorem}

\begin{theorem}
Given a graph of width $r$, there exists a $(1/2,1/4)$-cover of size $\mathcal{O}(r^2)$.
\end{theorem}

\section{Algorithm for graphs of bounded width}


We now describe the algorithm for computing small diameter decomposition for graphs of width $(r,r)$. Let $G=(V,E)$ be a graph of width $(r,r)$ with edge-capacity $c:E \rightarrow \mathds{R}_{\ge 0}$ and edge-length $l:E \rightarrow \mathds{R}_{\geq 0}$. Let $\mathcal{S}(G)=\{S_1,S_2,\ldots,S_t\}$ be the bag decomposition of $G$ and $T(G)$ be the corresponding rooted tree. Given a connected subgraph $G'=(V',E')$ of $G$, let $\mathcal{S}(G')=\{V' \cap S_1,V' \cap S_2,\ldots,V' \cap S_t\}$ and $T(G')$ be the (rooted) subtree of $T(G)$ on non-empty bags of $\mathcal{S}(G')$. It is easy to see that if $G'$ is connected, then so is $T(G')$. Let $t(G')$ denote the root bag of $T(G')$. 

Our algorithm runs in $r$ iterations. In iteration $i$, we pick a set of cuts using the region growing lemma such that the connected components of the graph obtained after removing the cut edges has width $(r-i,r)$. After $r$ iterations, we are left with connected components with width $(0,r)$. Connected components of width $(0,r)$ correspond precisely to the setting of Lemma \ref{lemma:sdd_width_0}, which we then use to find a small diameter decomposition. Next we describe our procedure $\cut(H)$, which given a graph $H$ of width $(j,r)$ outputs a graph of width $(j-1,r)$.

\textbf{Procedure cut($H$)}: Suppose we are given $H$ which is a subgraph of $G$ and has width $(j,r)$. Let $S$ be the root bag of $H$. Using the region growing lemma, we pick a radius $p \in [1/4,1/2)$ such that
\begin{equation*}
C(S,p) \leq 4 \cdot \log \left( \dfrac{V(S,1/2)}{V(S,1/4)} \right) \cdot V(S,p)
\end{equation*}
We set the value of $V(S,0)=F(S)/r$, where $F(S)=V(S,1/2)-V(S,0)$. Hence, $V(S,1/2)=F(S)/r+F(S), V(S,1/4) \geq F(S)/r$ and we have: 
\begin{equation*}
C(S,p)  \leq  4 \cdot \log (r+1) \cdot V(S,p) \leq  4 \cdot \log (r+1) \cdot V(S,p)   
\end{equation*}

Our algorithm follows the same general outline as the algorithm of Garg et al.~\cite{garg1996approximate}. Given a graph $G$, tree decomposition tree $T$ and a current multicut $\mathcal{M}$, we define a procedure $\cut(G)$ as follows: choose $p \sim \mathds{U}(1/4,1/2)$ and set $\mathcal{M}=\mathcal{M} \cup \delta(B(r(T),p)$.  



\begin{lemma} \label{lemma:algorithm_2r_bound}
Given a graph $G=(V,E)$ of treewidth $tw$ and a $(1/2,1/4)$-cover, each edge $e \in E$ can at most be in $2 \times tw$ sets of the cover.
\end{lemma}

\begin{proof}
Let $G=(V,E)$ be a graph with edge capacities $c:E \rightarrow \mathds{R}_{\geq 0}$ and edge lengths $l: E \rightarrow \mathds{R}_{\geq 0}$. Let $T(G)$ be one Tree decomposition of width $tw$ of graph $G$ and $t(G)$ the root of that tree. 

We consider the top most bag of the tree decomposition as the center of the first ball and expand it to a distance ${r_1 \sim \mathds{U}(\frac{1}{4},\frac{1}{2})}$ away from the center and downward in $T(G)$. We continue to create these balls by choosing as center the highest bag in $T(G)$ with no elements in another ball and ${r_i \sim \mathds{U}(\frac{1}{4},\frac{1}{2})}$ for the $i^{th}$ \ball until every bag has at least one element in a \ball. We then iterate this process by considering only the vertices that were not taken in any ball during the last iterations. This process takes at most $tw$ iterations to cover all vertices.

At each iteration, two center of two distinct \ball have a distance of at least $\frac{1}{4}$ and since we only consider the downward sub-tree every time we expand the ball two balls cannot intersect. Otherwise, \shadow of two balls can intersect in the case of one ball's shadow and only its shadow going to the next bag in $T(G)$ and so the next ball starting in this same bag and hence having an intersection of shadow and ball in one iteration. If one edge is included in this intersection, it will then be disregarded by the next ball formations since it is in one ball and will only be in the intersection of two shadows then. This can happen at most once for each edge at each iteration. 


\end{proof}



